Matlab routines for centrality in directed acyclic graphs

New Matlab functions for network centrality are introduced. Instead of the mean distance, the generalized mean distance is used. If closer relationships are prioritized, this closeness measure is also defined for unconnected graphs. Instead of distance to all nodes, distance to selected nodes is considered. Besides the vertical in- and out-closeness measures, horizontal cross-closeness is proposed.

==> cand1.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of winning the Nobel Prize.\label{tab:results}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Probit}\\
\hline
Female              &      -0.242         &       8.228         &      -0.113         &       3.252         \\
      &     (-0.33)         &      (1.82)         &     (-0.40)         &      (1.92)          \\
Distance to Nobel professors      &      1.233\sym{**} &       2.671\sym{*}  &       0.522\sym{**} &       1.253\sym{*}  \\
                    &      (3.03)         &      (2.16)         &      (2.99)         &      (2.20) \\
Distance to Nobel students            &       4.116\sym{***}&       10.94\sym{**} &       2.285\sym{***}&       5.027\sym{**} \\
                    &      (4.53)         &      (2.60)         &      (4.53)         &      (3.17)         \\
\hline
Individual fixed effects & No & Yes & No & Yes \\

Observations        &        4248         &        1827         &        4248         &        1827         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\textit{t} statistics in parentheses; \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)
\end{tablenotes}
\end{table}

==> candidates.tex <==
\begin{longtable}{r l r r r l c c}
\caption{Nobel laureates and candidates.} \label{tab:names} \\
\hline ID & name & birth & death & won & alma mater & JEL & source \\ \hline 
\endfirsthead

\multicolumn{8}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline ID & name & birth & death & won & alma mater & JEL & source \\ \hline 
\endhead

\hline \hline
\endlastfoot

\hline \multicolumn{8}{r}{{Continued on next page}} \\ \hline
\endfoot
1	&	Ragnar Frisch 	&	1895	&	1973	&	1969	&	Oslo	&	E	&	-	\\
2	&	Jan Tinbergen 	&	1903	&	1994	&	1969	&	Leiden	&	E	&	-	\\
3	&	Paul Samuelson 	&	1915	&	2009	&	1970	&	Harvard	&	C	&	-	\\
4	&	Simon Kuznets 	&	1901	&	1985	&	1971	&	Columbia	&	O	&	-	\\
5	&	John Hicks 	&	1904	&	1989	&	1972	&	Oxford	&	C	&	-	\\
6	&	Kenneth Arrow 	&	1921	&	2017	&	1972	&	Columbia	&	D	&	-	\\
7	&	Wassily Leontief 	&	1905	&	1999	&	1973	&	Berlin	&	C	&	-	\\
8	&	Gunnar Myrdal 	&	1898	&	1987	&	1974	&	Stockholm	&	E	&	-	\\
9	&	Friedrich Hayek 	&	1899	&	1992	&	1974	&	Vienna	&	P	&	-	\\
10	&	Tjalling Koopmans 	&	1910	&	1985	&	1975	&	Leiden	&	C	&	-	\\
11	&	Leonid Kantorovich 	&	1912	&	1986	&	1975	&	Leningrad	&	C	&	-	\\
12	&	Milton Friedman 	&	1912	&	2006	&	1976	&	Columbia	&	E	&	-	\\
13	&	Bertil Ohlin 	&	1899	&	1979	&	1977	&	Stockholm	&	F	&	-	\\
14	&	James Meade 	&	1907	&	1995	&	1977	&	Cambridge	&	F	&	-	\\
15	&	Herbert Simon 	&	1916	&	2001	&	1978	&	Chicago	&	L	&	-	\\
16	&	Theodore Schultz 	&	1902	&	1998	&	1979	&	Wisconsin	&	O	&	-	\\
17	&	Arthur Lewis 	&	1915	&	1991	&	1979	&	LSE	&	O	&	-	\\
18	&	Lawrence Klein 	&	1920	&	2013	&	1980	&	MIT	&	C	&	-	\\
19	&	James Tobin 	&	1918	&	2002	&	1981	&	Harvard	&	G	&	-	\\
20	&	George Stigler 	&	1911	&	1991	&	1982	&	Chicago	&	D	&	-	\\
21	&	Gerard Debreu 	&	1921	&	2004	&	1983	&	Paris	&	D	&	-	\\
22	&	Richard Stone 	&	1913	&	1991	&	1984	&	Cambridge	&	E	&	-	\\
23	&	Franco Modigliani 	&	1918	&	2003	&	1985	&	New School	&	G	&	-	\\
24	&	James Buchanan 	&	1919	&	2013	&	1986	&	Chicago	&	H	&	-	\\
25	&	Robert Solow 	&	1924	&		&	1987	&	Harvard	&	O	&	-	\\
26	&	Maurice Allais 	&	1911	&	2010	&	1988	&	Paris	&	D	&	-	\\
27	&	Trygve Haavelmo 	&	1911	&	1999	&	1989	&	Oslo	&	C	&	-	\\
28	&	Merton Miller 	&	1923	&	2000	&	1990	&	Johns Hopkins	&	G	&	-	\\
29	&	Harry Markowitz 	&	1927	&		&	1990	&	Chicago	&	G	&	-	\\
30	&	William Sharpe 	&	1934	&		&	1990	&	Los Angeles	&	G	&	-	\\
31	&	Ronald Coase 	&	1910	&	2013	&	1991	&	LSE	&	K	&	-	\\
32	&	Gary Becker 	&	1930	&	2014	&	1992	&	Chicago	&	D	&	-	\\
33	&	Douglas North 	&	1920	&	2015	&	1993	&	Berkeley	&	N	&	-	\\
34	&	Robert Fogel 	&	1926	&	2013	&	1993	&	Johns Hopkins	&	N	&	-	\\
35	&	John Harsanyi 	&	1920	&	2000	&	1994	&	Stanford	&	C	&	-	\\
36	&	John Nash 	&	1928	&	2015	&	1994	&	Princeton	&	C	&	-	\\
37	&	Reinhard Selten 	&	1930	&	2016	&	1994	&	Frankfurt	&	C	&	-	\\
38	&	Robert Lucas 	&	1937	&		&	1995	&	Chicago	&	E	&	-	\\
39	&	William Vickrey 	&	1914	&	1996	&	1996	&	Columbia	&	D	&	-	\\
40	&	James Mirrlees 	&	1936	&	2018	&	1996	&	Cambridge	&	D	&	-	\\
41	&	Myron Scholes 	&	1941	&		&	1997	&	Chicago	&	G	&	-	\\
42	&	Robert Merton 	&	1944	&		&	1997	&	MIT	&	G	&	-	\\
43	&	Amartya Sen 	&	1933	&		&	1998	&	Cambridge	&	D	&	-	\\
44	&	Robert Mundell 	&	1932	&	2021	&	1999	&	MIT	&	E	&	-	\\
45	&	Daniel McFadden 	&	1937	&		&	2000	&	Minnesota	&	C	&	-	\\
46	&	James Heckman 	&	1944	&		&	2000	&	Princeton	&	C	&	-	\\
47	&	George Akerlof 	&	1940	&		&	2001	&	MIT	&	D	&	-	\\
48	&	Michael Spence 	&	1943	&		&	2001	&	Harvard	&	D	&	-	\\
49	&	Joseph Stiglitz 	&	1943	&		&	2001	&	MIT	&	D	&	-	\\
50	&	Vernon Smith 	&	1927	&		&	2002	&	Harvard	&	D	&	-	\\
51	&	Daniel Kahneman 	&	1934	&		&	2002	&	Berkeley	&	D	&	-	\\
52	&	Clive Granger 	&	1934	&	2009	&	2003	&	Nottingham	&	C	&	-	\\
53	&	Robert Engle 	&	1942	&		&	2003	&	Cornell	&	C	&	-	\\
54	&	Edward Prescott 	&	1940	&		&	2004	&	Carnegie Mellon	&	E	&	-	\\
55	&	Finn Kydland 	&	1943	&		&	2004	&	Carnegie Mellon	&	E	&	-	\\
56	&	Thomas Schelling 	&	1921	&	2016	&	2005	&	Harvard	&	C	&	-	\\
57	&	Robert Aumann 	&	1930	&		&	2005	&	MIT	&	C	&	-	\\
58	&	Edmund Phelps 	&	1933	&		&	2006	&	Yale	&	E	&	-	\\
59	&	Leonid Hurwicz 	&	1917	&	2008	&	2007	&	LSE	&	D	&	-	\\
60	&	Eric Maskin 	&	1950	&		&	2007	&	Harvard	&	D	&	-	\\
61	&	Roger Myerson 	&	1951	&		&	2007	&	Harvard	&	D	&	-	\\
62	&	Paul Krugman 	&	1953	&		&	2008	&	MIT	&	F	&	-	\\
63	&	Oliver Williamson 	&	1932	&	2020	&	2009	&	Carnegie Mellon	&	H	&	-	\\
64	&	Elinor Ostrom 	&	1933	&	2012	&	2009	&	Los Angeles	&	Q	&	-	\\
65	&	Dale Mortensen 	&	1939	&	2014	&	2010	&	Carnegie Mellon	&	D	&	-	\\
66	&	Peter Diamond 	&	1940	&		&	2010	&	MIT	&	D	&	-	\\
67	&	Christopher Pissarides 	&	1948	&		&	2010	&	LSE	&	D	&	-	\\
68	&	Christopher Sims 	&	1942	&		&	2011	&	Harvard	&	M	&	-	\\
69	&	Thomas Sargent 	&	1943	&		&	2011	&	Harvard	&	M	&	-	\\
70	&	Lloyd Shapley 	&	1923	&	2016	&	2012	&	Princeton	&	C	&	-	\\
71	&	Alvin Roth 	&	1951	&		&	2012	&	Stanford	&	D	&	-	\\
72	&	Eugene Fama 	&	1939	&		&	2013	&	Chicago	&	G	&	-	\\
73	&	Robert Shiller 	&	1946	&		&	2013	&	MIT	&	F	&	-	\\
74	&	Lars Peter Hansen 	&	1952	&		&	2013	&	Minnesota	&	F	&	-	\\
75	&	Jean Tirole 	&	1953	&		&	2014	&	MIT	&	L	&	-	\\
76	&	Angus Deaton 	&	1945	&		&	2015	&	Cambridge	&	I	&	-	\\
77	&	Oliver Hart 	&	1948	&		&	2016	&	Princeton	&	D	&	-	\\
78	&	Bengt Holmstrom 	&	1949	&		&	2016	&	Stanford	&	D	&	-	\\
79	&	Richard Thaler 	&	1945	&		&	2017	&	Rochester	&	D	&	-	\\
80	&	William Nordhaus 	&	1941	&		&	2018	&	MIT	&	Q	&	-	\\
81	&	Paul Romer 	&	1955	&		&	2018	&	Chicago	&	O	&	-	\\
82	&	Abhijit Banerjee 	&	1961	&		&	2019	&	Harvard	&	O	&	-	\\
83	&	Michael Kremer 	&	1964	&		&	2019	&	Harvard	&	O	&	-	\\
84	&	Esther Duflo 	&	1972	&		&	2019	&	MIT	&	O	&	-	\\
85	&	Robert Wilson 	&	1937	&		&	2020	&	Harvard	&	D	&	-	\\
86	&	Paul Milgrom 	&	1948	&		&	2020	&	Stanford	&	D	&	-	\\
87	&	David Card 	&	1956	&		&	2021	&	Princeton	&	J	&	-	\\
88	&	Joshua Angrist 	&	1960	&		&	2021	&	Princeton	&	C	&	-	\\
89	&	Guido Imbens 	&	1963	&		&	2021	&	Brown	&	C	&	-	\\
90	&	Ludwig von Mises	&	1881	&	1973	&		&	Vienna	&	P	&	Clarivate	\\
91	&	Frank Knight	&	1882	&	1972	&		&	Cornell	&	D	&	Clarivate	\\
92	&	Alvin Hansen	&	1887	&	1975	&		&	Wisconsin	&	E	&	ad hoc	\\
93	&	Harold Hotelling	&	1895	&	1973	&		&	Princeton	&	C	&	Clarivate	\\
94	&	Oskar Morgenstern	&	1902	&	1977	&		&	Vienna	&	D	&	ad hoc	\\
95	&	Abba Lerner	&	1903	&	1982	&		&	LSE	&	D	&	ad hoc	\\
96	&	Joan Robinson	&	1903	&	1983	&		&	Cambridge	&	E	&	Clarivate	\\
97	&	Ester Boserup	&	1910	&	1999	&		&	Copenhagen	&	O	&	ad hoc	\\
98	&	Edith Penrose	&	1914	&	1996	&		&	Johns Hopkins	&	M	&	ad hoc	\\
99	&	Lionel McKenzie	&	1919	&	2010	&		&	Princeton	&	D	&	ad hoc	\\
100	&	William Baumol	&	1922	&	2017	&		&	LSE	&		&	Clarivate	\\
101	&	Gordon Tullock	&	1922	&	2014	&		&	Chicago	&	K	&	Clarivate	\\
102	&	William Meckling	&	1922	&	1998	&		&	Chicago	&	G	&	ad hoc	\\
103	&	Jacob Mincer	&	1922	&	2006	&		&	Columbia	&	J	&	ad hoc	\\
104	&	Henri Theil	&	1924	&	2000	&		&	Utrecht	&	C	&	ad hoc	\\
105	&	Harold Demsetz	&	1930	&	2019	&		&	Northwestern	&	K	&	Clarivate	\\
106	&	Israel Kirzner	&	1930	&		&		&	New York	&	L	&	Clarivate	\\
107	&	Wayne Fuller	&	1931	&		&		&	Iowa	&	C	&	Clarivate	\\
108	&	Dale Jorgenson	&	1933	& 2022 &		&	Harvard	&	E	&	Clarivate	\\
109	&	Jagdish Bhagwati	&	1934	&		&		&	MIT	&	F	&	Clarivate	\\
110	&	Anne Krueger	&	1934	&		&		&	Wisconsin	&	H	&	Clarivate	\\
111	&	Amos Tversky	&	1937	&	1996	&		&	Michigan	&	D	&	ad hoc	\\
112	&	Fischer Black	&	1938	&	1995	&		&	Harvard	&	G	&	ad hoc	\\
113	&	Martin Feldstein	&	1939	&	2019	&		&	Oxford	&	E	&	Clarivate	\\
114	&	Michael Jensen	&	1939	&		&		&	Chicago	&	G	&	Clarivate	\\
115	&	Soren Johansen	&	1939	&		&		&	Copenhagen	&	C	&	Clarivate	\\
116	&	Richard Posner	&	1939	&		&		&	Harvard	&	K	&	Clarivate	\\
117	&	Sam Peltzman	&	1940	&		&		&	Chicago	&	H	&	Clarivate	\\
118	&	Stewart Myers	&	1940	&		&		&	Stanford	&	G	&	Clarivate	\\
119	&	Guillermo Calvo	&	1941	&		&		&	Yale	&	E	&	ad hoc	\\
120	&	Evan Porteus	&	1942	&		&		&	Case	&	D	&	ad hoc	\\
121	&	Martin Weitzman	&	1942	&	2019	&		&	MIT	&	Q	&	Clarivate	\\
122	&	Robert Hall	&	1943	&		&		&	MIT	&	E	&	Clarivate	\\
123	&	Mark Granovetter	&	1943	&		&		&	Harvard	&	D	&	Clarivate	\\
124	&	Katarina Juselius	&	1943	&		&		&	Helsinki	&	C	&	Clarivate	\\
125	&	Robert Barro	&	1944	&		&		&	Harvard	&	E	&	Clarivate	\\
126	&	Avinash Dixit	&	1944	&		&		&	MIT	&	D	&	Clarivate	\\
127	&	David Hendry	&	1944	&		&		&	LSE	&	C	&	Clarivate	\\
128	&	Stephen Ross	&	1944	&	2017	&		&	Harvard	&	G	&	Clarivate	\\
129	&	Anthony Atkinson	&	1944	&	2017	&		&	Cambridge	&	D	&	Clarivate	\\
130	&	Brian Arthur	&	1945	&		&		&	Michigan	&	D	&	Clarivate	\\
131	&	David Dickey	&	1945	&		&		&	Iowa	&	C	&	Clarivate	\\
132	&	Jerry Hausman	&	1946	&		&		&	Oxford	&	C	&	Clarivate	\\
133	&	Elhanan Helpman	&	1946	&		&		&	Harvard	&	F	&	Clarivate	\\
134	&	Hashem Pesaran	&	1946	&		&		&	Cambridge	&	C	&	Clarivate	\\
135	&	John Taylor	&	1946	&		&		&	Stanford	&	E	&	Clarivate	\\
136	&	Claudia Goldin	&	1946	&		&		&	Chicago	&	J	&	Clarivate	\\
137	&	Francine Blau	&	1946	&		&		&	Harvard	&	J	&	ad hoc	\\
138	&	Joel Mokyr	&	1946	&		&		&	Yale	&	N	&	Clarivate	\\
139	&	Jean-Jacques Laffont	&	1947	&	2004	&		&	Harvard	&	L	&	ad hoc	\\
140	&	Edward Lazear	&	1948	&	2020	&		&	Harvard	&	J	&	Clarivate	\\
141	&	Olivier Blanchard	&	1948	&		&		&	MIT	&	E	&	Clarivate	\\
142	&	Peter Phillips	&	1948	&		&		&	LSE	&	C	&	Clarivate	\\
143	&	Charles Manski	&	1948	&		&		&	MIT	&	C	&	Clarivate	\\
144	&	David Teece	&	1948	&		&		&	Pennsylvania	&	L	&	Clarivate	\\
145	&	Ariel Pakes	&	1949	&		&		&	Harvard	&	C	&	Clarivate	\\
146	&	David Kreps	&	1950	&		&		&	Stanford	&	D	&	Clarivate	\\
147	&	Halbert White	&	1950	&	2012	&		&	MIT	&	C	&	Clarivate	\\
148	&	Ariel Rubinstein	&	1951	&		&		&	Jerusalem	&	C	&	Clarivate	\\
149	&	Mark Gertler	&	1951	&		&		&	Stanford	&	E	&	Clarivate	\\
150	&	Richard Blundell	&	1952	&		&		&	LSE	&	J	&	Clarivate	\\
151	&	Douglas Diamond	&	1953	&		&		&	Yale	&	G	&	Clarivate	\\
152	&	Kenneth Rogoff	&	1953	&		&		&	MIT	&	G	&	Clarivate	\\
153	&	Sanford Grossman	&	1953	&		&		&	Chicago	&	G	&	ad hoc	\\
154	&	John Moore	&	1954	&		&		&	LSE	&	G	&	Clarivate	\\
155	&	Kenneth French	&	1954	&		&		&	Rochester	&	G	&	Clarivate	\\
156	&	David Audretsch	&	1954	&		&		&	Wisconsin	&	L	&	Clarivate	\\
157	&	Gene Grossman	&	1955	&		&		&	MIT	&	F	&	Clarivate	\\
158	&	Nobuhiro Kiyotaki	&	1955	&		&		&	Harvard	&	G	&	Clarivate	\\
159	&	George Loewenstein	&	1955	&		&		&	Yale	&	D	&	Clarivate	\\
160	&	Carmen Reinhart	&	1955	&		&		&	Columbia	&	F	&	Clarivate	\\
161	&	Philippe Aghion	&	1956	&		&		&	Harvard	&	O	&	Clarivate	\\
162	&	Ernst Fehr	&	1956	&		&		&	Vienna	&	D	&	Clarivate	\\
163	&	Manuel Arellano	&	1957	&		&		&	LSE	&	C	&	Clarivate	\\
164	&	Daniel Levinthal	&	1957	&		&		&	Stanford	&	M	&	Clarivate	\\
165	&	Alberto Alesina	&	1957	&	2020	&		&	Harvard	&	H	&	Clarivate	\\
166	&	Kevin Murphy	&	1958	&		&		&	Chicago	&	D	&	Clarivate	\\
167	&	James Levinsohn	&	1958	&		&		&	Princeton	&	F	&	Clarivate	\\
168	&	Tim Bollerslev	&	1958	&		&		&	San Diego	&	C	&	IDEAS/RePEc	\\
169	&	John Campbell	&	1958	&		&		&	Yale	&	G	&	IDEAS/RePEc	\\
170	&	Stephen Berry	&	1959	&		&		&	Wisconsin	&	C	&	Clarivate	\\
171	&	Pierre Perron	&	1959	&		&		&	Yale	&	C	&	Clarivate	\\
172	&	Colin Camerer	&	1959	&		&		&	Chicago	&	D	&	Clarivate	\\
173	&	Robert Vishny	&	1959	&		&		&	MIT	&	G	&	IDEAS/RePEc	\\
174	&	Alan Krueger	&	1960	&	2019	&		&	Harvard	&	J	&	Clarivate	\\
175	&	Jordi Gali	&	1961	&		&		&	MIT	&	E	&	Clarivate	\\
176	&	Andrei Shleifer	&	1961	&		&		&	MIT	&	G	&	IDEAS/RePEc	\\
177	&	Stephen Bond	&	1963	&		&		&	Oxford	&	C	&	Clarivate	\\
178	&	Raghuram Rajan	&	1963	&		&		&	MIT	&	E	&	Clarivate	\\
179	&	Matthew Rabin	&	1963	&		&		&	MIT	&	D	&	Clarivate	\\
180	&	Daron Acemoglu	&	1967	&		&		&	LSE	&	O	&	IDEAS/RePEc	\\
181	&	Marc Melitz	&	1968	&		&		&	Michigan	&	F	&	Clarivate	\\
182	&	John List	&	1968	&		&		&	Wyoming	&	D	&	Clarivate	\\


\end{longtable}

==> candtable.tex <==
\begin{table}[htbp]\centering
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of winning the Nobel Prize with alternative fixed effects.\label{tab:fixed}}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}\\
\hline
Female              &      -1.015         &      -0.387         &      -1.032         &      -0.411         &      -1.705\sym{*}  &      -0.697\sym{*}  &      -1.039         &      -1.039         \\
                    &     (-1.41)         &     (-1.49)         &     (-1.43)         &     (-1.54)         &     (-2.11)         &     (-2.13)         &     (-1.39)         &     (-1.39)         \\
[1em]
Proximity to Nobel professors&       0.575         &       0.244         &       0.598         &       0.243         &       0.567         &       0.207         &       0.511         &       0.511         \\
                    &      (1.40)         &      (1.44)         &      (1.45)         &      (1.40)         &      (1.12)         &      (0.99)         &      (1.15)         &      (1.15)         \\
[1em]
Proximity to Nobel students&       3.322\sym{***}&       1.816\sym{***}&       3.713\sym{***}&       1.885\sym{***}&       5.017\sym{**} &       2.342\sym{**} &       3.858\sym{***}&       3.858\sym{***}\\
                    &      (4.19)         &      (4.08)         &      (3.54)         &      (3.76)         &      (3.26)         &      (3.12)         &      (3.35)         &      (3.35)         \\
\hline
Year fixed effects & No & No & Yes & Yes & Yes & Yes & Yes &  Yes\\
\textit{Alma mater} fixed effects & No & No & No & No & Yes & Yes & No & No \\
Field fixed effects & No & No & No & No & No & No & Yes & Yes\\
Individual fixed effects & No & No & No & No & No & No & No & No\\
Observations        &        4508         &        4508         &        4508         &        4508         &        3975         &        3975         &        4460         &        4460         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> candtabledist.tex <==
\begin{table}[htbp]\centering\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of winning the Nobel Prize for alternative measures of distance.\label{tab:distance}}
\begin{tabular}{l*{8}{c}}
\hline\hline
                   &\multicolumn{2}{c}{$p=-0.5$} &\multicolumn{2}{c}{$p=-1$}
                   &\multicolumn{2}{c}{$p=-2$}
                   &\multicolumn{2}{c}{$p=-1$}\\
                    &\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}\\
\hline
female              &      -1.099         &      -0.439         &      -1.032         &      -0.411         &      -0.953         &      -0.375   &      -0.982         &      -0.380 \\
                    &     (-1.53)         &     (-1.65)         &     (-1.43)         &     (-1.54)         &     (-1.32)         &     (-1.41)    &     (-1.36)         &     (-1.43)      \\
[1em]
Proximity to Nobel professors             &       0.234         &       0.101       &       0.598         &       0.243         &   0.568         &       0.228 &       0.236         &      0.0959                   \\
                     &      (0.41)         &      (0.42)      &      (1.45)         &      (1.40)         &         (1.70)         &      (1.64)    &      (0.53)         &      (0.52)      \\
[1em]
Proximity to Nobel students            &       1.822         &       0.958      &       3.713\sym{***}&       1.885\sym{***}&  3.869\sym{***}&       1.852\sym{***}   &       3.755\sym{***}&       1.890\sym{***}                \\
                    &      (1.09)         &      (1.14)        &      (3.54)         &      (3.76)         &                 (5.94)         &      (5.55) &      (3.60)         &      (3.77)         \\
                    [1em]
Proximity to Nobel siblings             &                     &                     &                     &                     &                     &                     &       1.131\sym{*}  &       0.500\sym{*}  \\
                    &                     &                     &                     &                     &                     &                     &      (2.48)         &      (2.54)         \\
\hline
\hline
Year fixed effects & Yes & Yes & Yes & Yes & Yes &  Yes & Yes &  Yes\\
\textit{Alma mater} fixed effects & No & No & No & No & No & No & No & No \\
Field fixed effects & No & No & No & No & No & No & No & No \\
Individual fixed effects & No & No & No & No & No & No  & No & No\\
Observations        &        4508         &        4508         &        4508         &        4508         &        4508         &        4508 &        4508         &        4508         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> candtablelimit.tex <==
\begin{table}[htbp]\centering\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of winning the Nobel Prize for alternative sets of candidates.\label{tab:who}}
\begin{tabular}{l*{8}{c}}
\hline\hline
 &\multicolumn{2}{c}{all} &\multicolumn{2}{c}{without ad hoc} &\multicolumn{2}{c}{without IDEAS/RePEc} &\multicolumn{2}{c}{Nobelists only} \\
 &\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}\\
\hline
Female              &      -1.032         &      -0.411         &      -0.777         &      -0.318         &      -0.813         &      -0.336         &       8.228         &       3.252         \\
                     &     (-1.43)         &     (-1.54)         &     (-1.08)         &     (-1.15)         &     (-1.13)         &     (-1.21)         &      (1.82)         &      (1.92)         \\
[1em]
Proximity to Nobel professors &       0.598         &       0.243         &       0.529         &       0.218         &       0.617         &       0.254         &       2.671\sym{*}  &       1.253\sym{*}  \\
                    &      (1.45)         &      (1.40)        &      (1.29)         &      (1.25)         &      (1.52)         &      (1.46)         &      (2.16)         &      (2.20)         \\
[1em]
Proximity to Nobel students &       3.713\sym{***}&       1.885\sym{***} &       3.511\sym{***}&       1.803\sym{***}&       3.506\sym{***}&       1.793\sym{***}&       10.94\sym{**} &       5.027\sym{**} \\
                    &      (3.54)         &      (3.76)          &      (3.35)         &      (3.57)         &      (3.36)         &      (3.55)         &      (2.60)         &      (3.17)         \\
\hline
Year fixed effect & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
\textit{Alma mater} fixed effects & No & No & No & No & No & No & No & No\\
Field fixed effects & No & No & No & No & No & No & No & No\\
Individual fixed effects & No & No & No & No & No & No & Yes & Yes\\
Observations        &        4508         &        4508         &        4091         &        4091         &        3989         &        3989         &        1827         &        1827         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> candtablesplit.tex <==
\begin{table}[htbp]\centering
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of winning the Nobel Prize for different types of Nobelists.\label{tab:living}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}\\
\hline
Female              &      -1.032         &      -0.411         &      -1.033         &      -0.408         &      -1.033         &      -0.408         \\
                    &     (-1.43)         &     (-1.54)         &     (-1.43)         &     (-1.53)         &     (-1.43)         &     (-1.53)         \\
[1em]
Proximity to Nobel students&       3.713\sym{***}&       1.885\sym{***}&       3.592\sym{***}&       1.833\sym{***}&       3.592\sym{***}&       1.833\sym{***}\\
                    &      (3.54)         &      (3.76)         &      (3.43)         &      (3.64)         &      (3.43)         &      (3.64)         \\
[1em]
Proximity to Nobel professors&       0.598         &       0.243         &                     &                     &                     &                     \\
                    &      (1.45)         &      (1.40)         &                     &                     &                     &                     \\
[1em]
Proximity to deceased Nobel professors&                     &                     &       0.955\sym{*}  &       0.417\sym{*}  &                     &                     \\
                    &                     &                     &      (2.07)         &      (2.04)         &                     &                     \\
[1em]
Proximity to living Nobel professors&                     &                     &       0.208         &      0.0820         &                     &                     \\
                    &                     &                     &      (0.50)         &      (0.48)         &                     &                     \\
[1em]
Proximity to earlier enNobeled professors&                     &                     &                     &                     &       0.955\sym{*}  &       0.417\sym{*}  \\
                    &                     &                     &                     &                     &      (2.07)         &      (2.04)         \\
[1em]
Proximity to recently enNobeled professors&                     &                     &                     &                     &       0.208         &      0.0820         \\
                    &                     &                     &                     &                     &      (0.50)         &      (0.48)         \\
\hline
Year fixed effect & Yes & Yes & Yes & Yes & Yes & Yes \\
\textit{Alma mater} fixed effects & No & No & No & No & No & No \\
Field fixed effects & No & No & No & No & No & No \\
Individual fixed effects & No & No & No & No & No & No\\
Observations        &        4508         &        4508         &        4508         &        4508         &        4508         &        4508         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}

